Graph Isomorphism for Graph Classes Characterized by two Forbidden Induced Subgraphs

We study the complexity of the Graph Isomorphism problem on graph classes that are characterized by a finite number of forbidden induced subgraphs, focusing mostly on the case of two forbidden subgraphs. We show hardness results and develop techniques for the structural analysis of such graph classes, which applied to the case of two forbidden subgraphs give the following results: A dichotomy into isomorphism complete and polynomial-time solvable graph classes for all but finitely many cases, whenever neither of the forbidden graphs is a clique, a pan, or a complement of these graphs. Further reducing the remaining open cases we show that (with respect to graph isomorphism) forbidding a pan is equivalent to forbidding a clique of size three.

==> conclusion.tex <==
% % \section{Conclusion}\label{sec:conclusion}
% % 
% % In order to initiate a systematic study of the \griso Problem on hereditary graph classes  we considered graph classes characterized by two forbidden induced subgraphs. From a series of reductions we obtain strong restrictions on the choice of forbidden subgraphs; unless one of the forbidden graphs simultaneously adheres to several of these restrictions, \griso remains GI-complete on the class of~$\forbind{H_1,H_2}$ graphs. 
% % We presented a complete characterization of the case that neither of the two forbidden subgraphs fulfills all split conditions into GI-complete and polynomial cases. For the other case, i.e., the case of one graph fulfilling all split conditions, we were able to reduce the open questions to classes where one forbidden subgraph behaves like an independent set (i.e., is basic) plus few concrete pairs of forbidden subgraphs.
% % % For the case in which one of the graphs is an independent set, our reductions and our polynomial-time algorithms are still applicable and have consequences for the second graph.
% % % \todo{The cases that are not covered appear} to be of different nature and their resolution shall be the next step for our systematic study. 
% % 
% % 
% % The polynomially-solvable cases from Section~\ref{sec:bothsplit} contain all graphs of some bounded degree. For such classes, the only known technique for a polynomial time algorithm is the one by Luks~\cite{Luks:1982}. It would thus be surprising if other known techniques could resolve them. However, for the finitely many unresolved cases, other techniques may be successful. In particular, many of these classes are of bounded clique-width and modular decomposition techniques apply. \todo{For such an approach~\cite{brand} may be of interest. This paper researches cliquewidth in relationship to forbidden subgraphs.} We also remark that in a preprint Rao~\cite{Rao} resolves the case~$\forbind{gem,co-gem}$.
% % 
% % Future steps for studying the hereditary graph classes include the resolution of the remaining cases and analysis of graph classes characterized by more than two forbidden subgraphs;
% % many of our results have also implications for these classes.
% % % \todo{mention FPT results?: Since Theorem~\ref{theorem:bothsplit:result} can also be applied to colored graphs, the corollary follows from the fixed-parameter tractability results with parameter distance to~$\forbind{H_1,\ldots,H_k}$ graphs in~\cite{KratschSchweitzer}.}





\section{Conclusion}\label{sec:conclusion}

In order to initiate a systematic study of the \griso Problem on hereditary graph classes  we considered graph classes characterized by two forbidden induced subgraphs. 
We presented an almost complete characterization of the case that neither of the two forbidden subgraphs is basic into GI-complete and polynomial cases, leaving only few pairs of forbidden subgraphs.
Theorem~\ref{theorem:bothsplit:result} constitutes the main technical contribution towards this result. Together with the tractability of~$\forbindONE{P_4}$ graphs (Theorem~\ref{theorem:hfree:dichotomy},~\cite{Corneil1981163}) it establishes the polynomially solvable cases. On the other hand suppose~$H_1$ and~$H_2$ are non-basic and~$\forbind{H_1,H_2}$ is not a polynomial-time solvable case of Theorems~\ref{theorem:hfree:dichotomy} or~\ref{theorem:bothsplit:result}. Then, \griso on the class of~$\forbind{H_1,H_2}$ graphs is GI-complete, unless for~$H_1$ and~$H_2$, or for~$\overline{H_1}$ and~$\overline{H_2}$, one of the graphs is in $\{ P_4\dunion K_1, K_2\dunion I_2, P_3\dunion I_2\}$, and the other graph has at most 7 vertices and is the complement of a union of at most 3 paths.

% Summarizing, \griso on the class of~$\forbind{H_1,H_2}$ graphs is polynomially solvable, if one of the graphs is a subgraph of the~$P_4$ and if the class~$\forbind{H_1,H_2}$ is a suclass of a class~$\forbind{H(0,b,c),\overline{H(0,b',c')}}$ with certain allowed combinations of~$b,b',c,c'$ which are described in Theorem~\ref{theorem:bothsplit:result}. 





%  and the other graph is in~$\{\overline{2K_2},\overline{2K_2\dunion K_1},\overline{P_3\dunion K_2},\overline{P_4\dunion K_1},\overline{P_5},\overline{P_5\dunion K_1},\overline{P_6},\overline{P_7}\}$, or this is true for the complements~$\overline{H_1}$ and~$\overline{H_2}$.



% A more careful but tedious variant of the proof of Theorem~\ref{thm:one:split:finite:cases} explicitly keeps track of the remaining open cases, and leads to the following: Suppose~$H_1$ and~$H_2$ are non-basic and~$\forbind{H_1,H_2}$ is not a polynomial-time solvable case of Theorems~\ref{theorem:hfree:dichotomy} or~\ref{theorem:bothsplit:result}. Then, \griso on the class of~$\forbind{H_1,H_2}$ graphs is GI-complete, unless for~$H_1$ and~$H_2$, one of the graphs is in $\{ P_4\dunion K_1, K_2\dunion I_2, P_3\dunion I_2\}$ and the other graph is in~$\{\overline{2K_2},\overline{2K_2\dunion K_1},\overline{P_3\dunion K_2},\overline{P_4\dunion K_1},\overline{P_5},\overline{P_5\dunion K_1},\overline{P_6},\overline{P_7}\}$, or this is true for the complements~$\overline{H_1}$ and~$\overline{H_2}$.

% It is easy to see that results in this paper further resolve some of these cases, in particular GI-completeness on~$\forbind{P_4\dunion K_1,K_4}$ (Theorem~\ref{theorem:reduction:gicomplete}). 


% Some results in this paper (e.g., Theorem~\ref{theorem:reduction:gicomplete}) immediately resolve some of these 24 cases. 

Several further cases, e.g., all cases involving the~$\overline{P_6}$ or the~$\overline{P_7}$, can be excluded by variants of the reduction used for Theorem~\ref{theorem:reduction:gicomplete}. Of the remaining cases, in a preprint, Rao~\cite{Rao} resolves positively the case~$\forbind{P_4\dunion K_1,\overline{P_4\dunion K_1}}$ and its subclasses;  %~$\forbind{gem,co-gem}$
similar (modular) decomposition techniques appear to apply to other cases as well. 
Several of the remaining cases are classes of bounded 
clique-width~\cite{brand}, which could indicate their tractability. 

% \todo{Furthermore, some of the classes are of bounded clique-width~\cite{brand}, and hence likely to be tractable as their structure is limited.}
For the case in which one of the forbidden graphs is basic, our reductions and our polynomial-time algorithms are still applicable and resolve a large portion of the cases.  However, as mentioned in the introduction, complete resolution appears to require new techniques.
Future steps for studying the hereditary graph classes include the resolution of the remaining cases and analysis of graph classes characterized by more than two forbidden subgraphs.
% many of our results also have implications for these classes.

% Future steps for studying the hereditary graph classes include the resolution of the remaining cases and analysis of graph classes characterized by more than two forbidden subgraphs; many of our results also have implications for these classes.

